Sublinear Space Graph Algorithms in the Continual Release Model

The graph continual release model of differential privacy seeks to produce differentially private solutions to graph problems under a stream of edge updates where new private solutions are released after each update. Thus far, previously known edge-differentially private algorithms for most graph problems including densest subgraph and matchings in the continual release setting only output real-value estimates (not vertex subset solutions) and do not use sublinear space. Instead, they rely on computing exact graph statistics on the input [FHO21,SLMVC18]. In this paper, we leverage sparsification to address the above shortcomings for edge-insertion streams. Our edge-differentially private algorithms use sublinear space with respect to the number of edges in the graph while some also achieve sublinear space in the number of vertices in the graph. In addition, for the densest subgraph problem, we also output edge-differentially private vertex subset solutions; no previous graph algorithms in the continual release model output such subsets. We make novel use of assorted sparsification techniques from the non-private streaming and static graph algorithms literature to achieve new results in the sublinear space, continual release setting. This includes algorithms for densest subgraph, maximum matching, as well as the first continual release $k$-core decomposition algorithm. We also develop a novel sparse level data structure for $k$-core decomposition that may be of independent interest. To complement our insertion-only algorithms, we conclude with polynomial additive error lower bounds for edge-privacy in the fully dynamic setting, where only logarithmic lower bounds were previously known.

==> todos.tex <==
\begin{CheckList}{Task}
    \Task{done}{(Quanquan) Fix the approximation proof for insertion-only densest subgraphs.}
    \Task{done}{(Quanquan) Add default SVT whp guarantees as a lemma.}
    \Task{started}{(Tamalika) 
    Make a smoothed sensitivity based analysis
    for insertion-only streams. Can we use sublinear
    space algorithms with the smoothed sensitivity analysis?}
    \Task{started}{(Felix) Check and verify vertex cover analysis. 
    Make vertex cover analysis work for semi-streaming
    insertion-only setting.}
    \Task{started}{(Felix) private boosting algorithm.}
    \Task{open}{(See below) Other examples of algorithms that fit under our setting (i.e.\ low space, sparsification approaches)?}
        \begin{CheckList}{Task}
            \Task{open}{There is a difference between algorithms that return a subgraph as a solution and 
            those that only return a numerical value.}
            \Task{open}{For solutions that return only a numerical value, we can use the smooth sensitivity analysis.}
            \Task{open}{For solutions that return an actual subgraph, we need to adapt the techniques for each algorithm.}
            \Task{open}{\st{Update: nope; seems difficult for now...It would be good to be able to generalize some of the techniques we have for each of the algorithms above.}}
        \end{CheckList}
    \Task{open}{(?) Read over and polish fully dynamic, lazy-updates section (i.e.\ section where we delay release of a solution after
    a certain number of updates like doing lazy updates for dynamic graph problems)}
        \begin{CheckList}{Task}
            \Task{open}{(?) Can probably make it work for outputting a subgraph
            solution for a problem using static differentially private algorithm.}
            \Task{open}{Can potentially make smoothed sensitivity framework work with the lazy
            updates method.}
            \Task{open}{Note: fully dynamic probably not low space.}
            \Task{open}{\textbf{Needs problems that fit under the framework also}}
        \end{CheckList}
    \Task{open}{(?) Additional problems to check and consider:}
    \begin{CheckList}{Task}
        \Task{open}{Smoothed sensitivity analysis (potentially); these problems only output the size of the solution and not the solution
        itself: (more problems listed here: https://people.cs.umass.edu/~mcgregor/papers/13-graphsurvey.pdf and 
        in the corresponding slides \url{https://simons.berkeley.edu/sites/default/files/docs/928/mcgregorslides.pdf}) \tnote{double check about input parameters that may be sensitive}}
                \begin{CheckList}{Task}
                    \Task{open}{Can we make this framework also use privacy
                    amplification via subsampling? A lot of these algorithms are
                    actually sublinear in number of vertices for certain 
                    parameters.}
                    \Task{open}{\url{https://people.cs.umass.edu/~mcgregor/papers/13-graphsurvey.pdf}}
                    \Task{started}{(Quanquan) Maximum matching $(2+\alpha)(1+\eps)$ approximation: \url{https://people.cs.umass.edu/~mcgregor/papers/18-sosa.pdf};
                    requires arboricity $\alpha$}
                    \Task{open}{All the problems here probably have insertion-only streaming algorithms to estimate the sizes:
                    \url{https://arxiv.org/pdf/2106.14756.pdf}.}
                    \Task{open}{(?) \textbf{Cut sparsifiers} 
                    analyze smoothed sensitivity of Ahn and Guha's cut sparsifier: \url{https://arxiv.org/pdf/0902.0140.pdf}.}
                \end{CheckList}
        \Task{done}{(Nothing else works for now :'( ) Use the same strategy as our densest subgraph problem: a) use exact value to determine whether to output new answer b) output new answer using differentially private graph algorithm}
        \begin{CheckList}{Task}
            \Task{done}{(Quanquan) Streaming $k$-core decomposition: combine uniform sampling with \url{https://arxiv.org/abs/2106.03824}}
        \end{CheckList}
    \end{CheckList}
    \Task{done}{(Quanquan) Generalize our insertion-only framework for densest subgraphs to other problems (see above). Update: I wrote a 
    section but even for privacy, it is difficult to generalize the framework; thus, there is just a section of ``general principles''
    and no proofs.}
    \begin{enumerate}
        \item Show insertion-only resampling argument works under noisy probability distributions
        \item Use SVT to determine noisy probability distribution and when to update answer
        \item Update answer using private algorithm
    \end{enumerate}
    \Task{open}{(?) Additive lower bounds in dynamic streams for each problem we have an algorithm for in the insertion-only setting.}
\end{CheckList}

\felixnote{TODO: Big O' Table of Results!}

